Query-driven Data Completeness Management (PhD Thesis)

Knowledge about data completeness is essentially in data-supported decision making. In this thesis we present a framework for metadata-based assessment of database completeness. We discuss how to express information about data completeness and how to use such information to draw conclusions about the completeness of query answers. In particular, we introduce formalisms for stating completeness for parts of relational databases. We then present techniques for drawing inferences between such statements and statements about the completeness of query answers, and show how the techniques can be extended to databases that contain null values. We show that the framework for relational databases can be transferred to RDF data, and that a similar framework can also be applied to spatial data. We also discuss how completeness information can be verified over processes, and introduce a data-aware process model that allows this verification.

==> files/titleplain.tex <==
\newgeometry{margin=2cm}

\begin{titlepage}

 \newcommand{\HRule}{\rule{\linewidth}{0.5mm}}\pagenumbering{gobble}

\begin{center}
% Upper part of the page. The '~' is needed because \\
% only works if a paragraph has started.
~\\[1cm]
\par\end{center}

\begin{center}
\includegraphics[width=0.66\textwidth]{files/FUB-logo}~\\[2.4cm]
\par\end{center}

\begin{center}
\textsc{\Large{}PhD Thesis}{\Large{}\\[1.2cm]}
\par\end{center}{\Large \par}

\begin{center}
% Title
\HRule \\[0.4cm] { \textbf{\huge{}Query-driven Data Completeness
Management \\[0.4cm] }}
\par\end{center}{\huge \par}

\begin{center}
\HRule \\[1.5cm]
\par\end{center}

\begin{center}
% Author and supervisor
\begin{minipage}[c]{0.4\textwidth}%
 

\begin{flushleft}
\emph{\large{}Author:}{\large{}}\\
{\large{} Simon Razniewski }
\par\end{flushleft}%
\end{minipage}%
\begin{minipage}[c]{0.4\textwidth}%
 

\begin{flushright}
\emph{\large{}Supervisor:}{\large{} }\\
{\large{} Prof. Werner Nutt }
\par\end{flushright}%
\end{minipage}
\par\end{center}

\begin{center}
\vfill{}

\par\end{center}

\begin{center}
% Bottom of the page
{\large{}\today}
\par\end{center}{\large \par}

\end{titlepage}

\restoregeometry

\newpage{}


==> source_iswc/macros_iswc.tex <==


% This switches the style of most operators
%\newcommand{\ourStyle}[1]{{\small\texttt{#1}}}
\newcommand{\ourStyle}[1]{{\small\texttt{#1}}}


%%%%%%%%%%%%% Ario's Macros %%%%%%%%%%%%%


\newcommand{\itl}[1]{\textit{#1}}
\newcommand{\bo}[1]{\textbf{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\bi}[1]{\textbf{\textit{#1}}}
\newcommand{\m}[1]{\boldmath{\( #1 \)}}
%\newcommand{\code}[1]{{\ttfamily #1}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\rarw}{\rightarrow}
\newcommand{\ld}{\lambda}
\newcommand{\rw}{\rightarrow}
\newcommand{\ml}{\mathcal}

\newcommand{\sq}{\hbox{$\sqcap$\llap{$\sqcup$}}}
\newcommand{\lbsq}{\hbox{\rlap{$\blacksquare$}}}

%fariz added this
\newcommand{\leftouterjoin}{\; \includegraphics[scale=0.8]{ljoin.eps} \;}

%%%%%%%%%%%%% Simon's Macros %%%%%%%%%%%%%

\newcommand{\Null}{\textsl{null}\xspace}
\newcommand{\Nulls}{\textsl{null}s\xspace}
\newcommand{\pdb}{{\mathcal D\xspace}\xspace}
\newcommand{\D}{{\pdb}}
\newcommand{\id}[1]{#1^i}
\newcommand{\av}[1]{#1^a}
\newcommand{\epos}[2]{\textit{EPos}(#1,#2)}						% essential positions of a query
\newcommand{\etal}{et al.}
\newcommand{\satisfies}{\models}
\newcommand{\RQ}{\ensuremath{\L_{\rm{RQ}}}}
\newcommand{\CQ}{\ensuremath{\L_{\rm{CQ}}}}
\newcommand{\LRQ}{\ensuremath{\L_{\rm{LRQ}}}}
\newcommand{\LCQ}{\ensuremath{\L_{\rm{LCQ}}}}
\renewcommand{\L}{{\mathcal L}}									% used for query languages
\newcommand{\compl}[1]{\mathit{Compl}(#1)}
\newcommand{\complpi}[1]{\mathit{Compl}_{\pi}\ensuremath{(#1)}}
%\newcommand{\card}[1]{|#1|}
\newcommand{\localComp}{table completeness\xspace}
\newcommand{\LocalComp}{Table completeness\xspace}
\newcommand{\LC}{TC\xspace}
\newcommand{\LCQC}{\ensuremath{\mathsf{TC\text{-}QC}}}
\newcommand{\LCLC}{\ensuremath{\mathsf{TC\text{-}TC}}}
\newcommand{\QCQC}{\ensuremath{\mathsf{QC\text{-}QC}}}
\newcommand{\PTIME}{\ensuremath{\mathsf{PTIME}}}
\newcommand{\CONP}{\ensuremath{\mathsf{coNP}}}
\newcommand{\NP}{\ensuremath{\mathsf{NP}}}
\newcommand{\Cont}{\ensuremath{\mathsf{Cont}}}
\newcommand{\ContU}{\ensuremath{\mathsf{ContU}}}

%%%%%%%%%%%%% Basic Math Notations %%%%%%%%%%%%%

\newcommand{\eset}{\emptyset}
\newcommand\bigset[1]{ \Bigl\{ #1 \Bigr\} }   							% makes the big set { #1 }
\newcommand\bigmid{\ \Big|\ }
\newcommand{\incl}{\subseteq}
\newcommand{\incls}{\supseteq}
\newcommand{\col}{\colon}
\newcommand{\angles}[1]{\langle#1\rangle}       						% pointed angles

%%%%%%%%%%%%% Useful Bits and Pieces %%%%%%%%%%%%%

\newcommand{\dd}[2]{#1_1,\ldots,#1_{#2}}      							% da da, makes x1,...,xn
\newcommand{\quotes}[1]{\lq\lq#1\rq\rq}         						% makes ``#1''
\newcommand{\wrt}{w.r.t.\ }                        						% with respect to 
\newcommand{\WLOG}{wlog\xspace}                     					% without loss of generality
\newcommand{\Sum}{\ensuremath{{\sf sum}}}
\newcommand{\Count}{\ensuremath{{\sf count}}}
\newcommand{\Max}{\ensuremath{{\sf max}}}
\newcommand{\Min}{\ensuremath{{\sf min}}}
\newcommand\core[1]{\mathring{#1}}

%%%%%%%%%%%%% Renamings %%%%%%%%%%%%%

\newcommand{\qif}{\,{:}{-}\,}
\newcommand{\union}{\cup}
\newcommand{\lit}[1]{L_{#1}}
\newcommand{\cpred}[1]{V_{#1}}
\newcommand{\concond}{G}
\newcommand{\da}{\av D}
\newcommand{\di}{\id D}
\newcommand{\lcstmt}{C}
\newcommand{\cplstmt}[2]{#1 {\, \dot{\subseteq} \, } #2}
\newcommand{\Compl}[1]{\mathit{Compl}{(}#1{)}}
\newcommand{\Complb}[1]{\mathit{Compl}^b($#1$)}
\newcommand{\Compls}[1]{\mathit{Compl}^s($#1$)}
\newcommand{\Complsred}[1]{\mathit{Compl}^{sred}($#1$)}
\newcommand{\qcompl}[1]{\mathit{Compl}{(}#1{)}}
\newcommand{\cplset}{{\mathcal C}}
\newcommand{\Q}{{\mathcal Q}}                       				% used for set of queries
\newcommand{\F}{{\mathcal F}}                       				% used for set of finite domain constraints
\renewcommand{\S}{{\mathcal S}}                       				% used for sets of statements
\newcommand{\cplhat}{\hat C}
\newcommand{\chk}{\check}
% \renewcommand{\implies}{\rightarrow}
% \renewcommand{\And}{\wedge}
\newcommand{\Or}{\vee}
\newcommand{\findom}[3]{\mathit{Dom}(#1,#2,#3)} 					%Says which relation has which finite domain for which condition
\newcommand{\determines}{\rightarrow \! \! \! \! \! \rightarrow} 	%the determinacy symbol for query determinacy
\newcommand{\dotequiv}{\ \dot{\equiv} \ } 							%equivalence with dot, used in proof of boolean queries determinacy, completeness relation
\newcommand{\Wlog}{W.l.o.g.\ }
\newcommand{\ie}{i.\ e.\ ,}
\newcommand{\piptwo}{\Pi^P_2}
\newcommand{\sigptwo}{\Sigma^P_2}
\newcommand{\queryset}{{\mathcal Q}} 								% a set of queries
\newcommand{\schemaconstraintset}{{\mathcal F}} 					% a set of schema constraints
\newcommand{\scset}{\schemaconstraintset} 							%short form of the makro above
\newcommand{\qset}{\queryset}
\newcommand{\val}{\upsilon}
\newcommand{\viewset}{{\mathcal V}}
\newcommand{\tpl}[1]{\bar{#1}}										%make tuple
\newcommand{\tplsub}[2]{{\bar{#1}}_{#2}}							%make tuple
% \newcommand{\query}[2]{#1 \qif #2} 									%$\query{Q(\tpl x)}{B_1, .., B_n}$.
\newcommand{\aufz}[2]{#1_1,\ldots,#1_{#2}}    						% aufz x n, makes x1,...,xn
\newcommand{\Onlyif}{\lq\lq$\Rightarrow$\rq\rq\ \ }   				% 1st direction of iff-proof
\newcommand{\If}{\lq\lq$\Leftarrow$\rq\rq\ \ }        				% 2nd direction of iff-proof
\newcommand{\eat}[1]{}
\newcommand{\modelsms}{\models \! \! ^{\mathit{M \! \! S}}}		  	% turnstyle for multiset semantics
\newcommand{\joininquotes}{\mbox{ ``$\bowtie$"}}      				% a join in quotes used for describing the query corresponding to local completeness statements


%%%%%%%%%%%%% Tables and Attributes %%%%%%%%%%%%%

\newcommand{\student}{\texttt{student}\xspace}
\newcommand{\sid}{\texttt{sid}\xspace}
\newcommand{\name}{\texttt{name}\xspace}
\newcommand{\level}{\texttt{level}\xspace}
\newcommand{\hometown}{\texttt{hometown}\xspace}
\newcommand{\formTeacher}{\texttt{formTeacher}\xspace}
\newcommand{\viceFormTeacher}{\texttt{viceFormTeacher}\xspace}
\newcommand{\profile}{\texttt{profile}\xspace}
\newcommand{\customer}{\texttt{customer}}
\newcommand{\street}{\texttt{street}}
\newcommand{\city}{\texttt{city}}
\newcommand{\supplier}{\texttt{supplier}}
\newcommand{\partner}{\texttt{partner}}
\newcommand{\longTerm}{\texttt{long\_term}}
\newcommand{\contact}{\texttt{contact}}
\newcommand{\iD}{\texttt{id}}
\newcommand{\tcqc}{\ensuremath{\mathsf{TC\text{-}QC}}}
\global\long\def\mytpl#1{\langle#1\rangle}
\global\long\def\fc{f_{\C}}
\global\long\def\uk{\mathrm{uk}}
\global\long\def\na{\mathrm{n/a}}
\global\long\def\const{\mathrm{const}}
\global\long\def\codd{\mathrm{Codd}}
\global\long\def\sql{\mathrm{SQL}}
\global\long\def\can{\mathrm{can}}
\global\long\def\sred{\mathrm{sred}}
\global\long\def\complsred#1{\mathit{Compl^{\sred}}(#1)}
\global\long\def\complb#1{\mathit{Compl^{b}}(#1)}
\global\long\def\compls#1{\mathit{Compl^{s}}(#1)}
\global\long\def\complstar#1#2{\mathit{Compl}^{#2}(#1)}
\global\long\def\smixed{\mathrm{s+}}
\global\long\def\pdb{\mathcal{D}}
\global\long\def\domby{\preceq}
\global\long\def\dominates{\succeq}
\global\long\def\tpl#1{\bar{#1}}
\global\long\def\ctle{\mathbf{E}}
\global\long\def\ctlf{\mathbf{F}}
\global\long\def\ctla{\mathbf{A}}
\global\long\def\ctlg{\mathbf{G}}
\global\long\def\muexists{<\negthickspace\negthinspace-\negthickspace\negthinspace>}
\global\long\def\muall{[\negthinspace-\negthinspace]}
% \textit{}\global\long\def\statedescriptor{\mathrm{stateDescriptor}}
\global\long\def\mulp{\mu\mathcal{L_{\mathit{P}}}}
\global\long\def\mula{\mu\mathcal{L_{\mathit{A}}}}
\global\long\def\live{\mathrm{Live}}
\global\long\def\chase{\mathrm{chase}}
\newcommand{\todo}[1]{\textcolor{red}{\textsl{Todo: #1}}}
\newcommand{\OnlyIf}{\lq\lq$\Rightarrow$\rq\rq\ \ }
\newcommand{\NULL}{\bot}
\newcommand{\arity}[1]{\textit{arity}(#1)}
\renewcommand{\student}{\ensuremath{\mathtt{student}}\xspace}
\newcommand{\classCode}{\ensuremath{\mathtt{classCode}}\xspace}
\renewcommand{\name}{\ensuremath{\mathtt{name}}\xspace}
\newcommand{\homeTown}{\ensuremath{\mathtt{homeTown}}\xspace}
%\renewcommand{\code}{\ensuremath{\mathtt{code}}\xspace}
\newcommand{\hascode}{\ensuremath{\mathtt{hasCode}}\xspace}
\renewcommand{\profile}{\ensuremath{\mathtt{profile}}\xspace}
\renewcommand{\formTeacher}{\ensuremath{\mathtt{formTeacher}}\xspace}
\newcommand{\lncourse}{\ensuremath{\mathtt{lnCourse}}\xspace}
\newcommand{\hasattr}{\ensuremath{\mathtt{hasAttr}}\xspace}
\newcommand{\attr}{\ensuremath{\mathtt{attr}}\xspace}
\newcommand{\arts}{\mathrm{'arts'}\xspace}
\newcommand{\school}{\textit{school}\xspace}
\newcommand{\Mary}{\mathrm{Mary}}
\newcommand{\Paul}{\mathrm{Paul}}
\newcommand{\Chester}{\mathrm{Chester}}
\newcommand{\Hampton}{\mathrm{Hampton}}
\newcommand{\twoA}{\mathrm{2a}}
\renewcommand{\qif}{\leftarrow}
\newcommand{\nonulls}[1]{{#1}^{\downarrow}}
\newcommand{\nonullsmod}[1]{{#1}^{\Downarrow}} 
\newcommand{\Rule}[1]{\rho_{#1}}
\newcommand{\tcruleEx}[3]{{#1}\rightarrow \exists\,{#2}{\mbox{\bf .}}\,{#3}}
\newcommand{\tcrule}[2]{{#1}\rightarrow{#2}}
\newcommand{\IF}{\mathrm{inc}}
\newcommand{\RF}{\mathrm{res}}
\newcommand{\PF}{\mathrm{2\bot}}
\newcommand{\TN}{\mathrm{3\bot}}
\newcommand{\AN}{\mathrm{ambg}}
\newcommand{\cert}{\mathrm{cert}}
\renewcommand{\chase}{\ensuremath{\mathit{chase}}\xspace}
\newcommand{\SIG}{\Sigma}
\newcommand{\SIGi}{\id{\SIG}}
\newcommand{\SIGa}{\av{\SIG}}

%---------------------------------------------------------------------------------
% MACROS FOR QUERY COMPLETENESS OVER LINKED DATA
%---------------------------------------------------------------------------------

\newcommand{\set}[1]{\{\,#1\,\}} 								% from Simon
\newcommand{\mathSet}[1]{\ensuremath{\{\,#1\,\}}}
\newcommand{\bag}[1]{\{\hspace{-0.13em}|\, #1 \,|\hspace{-0.13em}\}}   		% bag notation

\newcommand{\Ga}{\ensuremath{G^a}} 							% available graph
\newcommand{\Gi}{\ensuremath{G^i}} 							% ideal/complete graph

\newcommand{\QC}{\ensuremath{\mathit{Compl}(Q)}} 		% QC statement in general

\newcommand{\buildQC}[1]{\ensuremath{\mathit{Compl}(\mathit{#1})}}
\newcommand{\buildQCset}[1]{\ensuremath{\mathit{Compl}^s(\mathit{#1})}}
\newcommand{\buildQCbag}[1]{\ensuremath{\mathit{Compl}^b(\mathit{#1})}}

\newcommand{\defineGC}[2]{\ensuremath{\mathit{Compl}(#1 \mid #2)}}
\newcommand{\defineGCone}[1]{\ensuremath{\mathit{Compl}(#1)}}

\newcommand{\buildGC}[2]{\ensuremath{\mathit{Compl}(\set{#1} \mid \set{#2})}}
\newcommand{\buildGCone}[1]{\ensuremath{\mathit{Compl}(\set{#1})}}

\newcommand{\calC}{\ensuremath{\mathcal{C}}} 				% used to represent a set of GC statements
\newcommand{\GCC}{\calC} 	

\newcommand{\term}[1]{\ensuremath{\mathtt{#1}}}

\newcommand\mytabs{\hspace*{2\parindent}\=\hspace{1cm}\=\hspace{1cm}\=\hspace{1cm}\=\hspace{1cm}}
\newenvironment{mytabbing}[1][\mytabs]
  {\begin{tabbing}#1\kill}
  {\end{tabbing}}

% all SPARQL queries builder
\newcommand{\defineASK}[1]			{\ensuremath{(\ourStyle{ASK} \; #1)}}
\newcommand{\buildASK}[1]			{\ensuremath{(\ourStyle{ASK} \; \mathSet{#1})}}
\newcommand{\defineSELECT}[2]		{\ensuremath{(\ourStyle{SELECT} \; #1 \; #2)}}
\newcommand{\buildSELECT}[2]		{\ensuremath{(\ourStyle{SELECT} \; \mathSet{#1} \; \mathSet{#2})}}
\newcommand{\defineCONSTRUCT}[2]	{\ensuremath{(\ourStyle{CONSTRUCT} \; #1 \; #2)}}
\newcommand{\buildCONSTRUCT}[2]		{\ensuremath{(\ourStyle{CONSTRUCT} \; \{\mathSet{#1}\} \; \{\mathSet{#2}\})}}

\newcommand{\ASK}			{\ourStyle{ASK}\xspace}
\newcommand{\SELECT}		{\ourStyle{SELECT}\xspace}
\newcommand{\CONSTRUCT}		{\ourStyle{CONSTRUCT}\xspace}
\newcommand{\DISTINCT}		{\ourStyle{DISTINCT}\xspace}
\newcommand{\UNION}		{\ourStyle{UNION}\xspace}
\newcommand{\FILTER}	{\ourStyle{FILTER}\xspace}
\newcommand{\OR}	{\ourStyle{OR}\xspace}
\newcommand{\MINUS}	{\ourStyle{MINUS}\xspace}


\newcommand{\map}[2]{\ensuremath{\text{#1} \mapsto \text{#2}}}
\newcommand{\triple}[3]{(\mathit{#1}, \mathit{#2}, \mathit{#3})}

\newcommand{\buildIFF}[2]{\ensuremath{#1 \;\;\;\; \text{iff} \;\;\;\; #2}}

\newcommand{\evalset}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}^s}}
\newcommand{\evalbag}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}^b}}
\newcommand{\evalsetbag}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}}}
\newcommand{\eval}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}}}
\newcommand{\card}		[3]		{\ensuremath{\mathit{card}_{\evalbag{#1}{#2}}(#3)}}		%1: graph pattern, 2: graph, 3: mapping
\newcommand{\cardMapping}	[2]		{\ensuremath{\mathit{card}_{#1}(#2)}}						%1: mapping bag, 2: mapping

\newcommand{\var}[1]{\ensuremath{\mathit{var}(#1)}}
\newcommand{\vars}[1]{\ensuremath{\mathit{vars}(#1)}}
\newcommand{\dom}[1]{\ensuremath{\mathit{dom}(#1)}}

% macros w/o parameters
\newcommand{\emptymap}		{\ensuremath{\mu_{\emptyset}}}
\newcommand{\mappingset}	{\ensuremath{\Omega}}
\newcommand{\rhodf}			{\ensuremath{\rho \mathit{DF}}}
\newcommand{\cl}				{\ensuremath{\mathit{cl}}}
\newcommand{\alphaVersion} 	{{\color{red} ALPHA VERSION!!!}}

\newcommand{\true}			{\texttt{true}\xspace}
\newcommand{\false}			{\texttt{false}\xspace}

\newcommand{\Graph}{\ensuremath{G}}
\newcommand{\Pattern}{\ensuremath{P}}

% DB stuff
\newcommand{\buildDBQuery}[2]{\ensuremath{{#1}\;\text{:-}\;{#2}}}

% federated query stuff
\newcommand{\calF}{\ensuremath{\mathcal{F}}} 				% used to represent a set of data sources
\newcommand{\fed}			[1]		{\ensuremath{\mathit{fed}_\calF(#1)}}
\newcommand{\evalfed}	[2]		{\ensuremath{\llbracket \fed{#1} \rrbracket_{#2}^s}}
\newcommand{\evalfedset}	[1]		{\ensuremath{\llbracket \fed{#1} \rrbracket_{\emptyset}^s}}
\newcommand{\defineSERVICE}[2]		{\ensuremath{(\ourStyle{SERVICE} \; #1 \; #2)}}

% OPT stuff
\newcommand{\subsumedBy}{\sqsubseteq}
\newcommand{\lessInformativeThan}{\subsumedBy}
\newcommand{\buildSELECTnew}[2]		{\ensuremath{(\mathit{SELECT} \; \mathSet{#1} \; #2)}}
%\newcommand{\OPT} {$\;$ OPT $\;$}
	\DeclareMathOperator{\OPT}{\ourStyle{OPT}}
\newcommand{\newvars}			[1]		{\ensuremath{\mathit{newvars}(#1)}}
\newcommand{\ext}			[1]		{\ensuremath{\mathit{ext}(#1)}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}} 				% used to represent trees

\newcommand{\evaltopdown}	[2]		{\ensuremath{\llbracket #1 \rrbracket^{td}_{#2}}}

% QUERY GENERATOR
\newcommand{\queryMINUS} [2] {(#1 \ourStyle{ MINUS } #2)}
\newcommand{\queryUNION} [2] {(#1 \ourStyle{ UNION } #2)}
\newcommand{\queryAND} [2] {(#1 \ourStyle{ AND } #2)}
\newcommand{\queryOPT} [2] {(#1 \ourStyle{ OPT } #2)}
\newcommand{\queryFILTER} [2] {(#1 \ourStyle{ FILTER } #2)}
\newcommand{\querySERVICE} [2] {(\ourStyle{SERVICE} \; #1 \; #2)}
\newcommand{\querySERVICEBraces} [2] {(\ourStyle{SERVICE} \; #1 \; \{#2\})}


\newcommand{\code}	[1] {\texttt{#1}}
\newcommand{\yes} {\texttt{yes}}
\newcommand{\notexists}	[1]	{\ensuremath{\ourStyle{NOT} \; \ourStyle{EXISTS}}(#1)}

\newcommand{\iri}			[1]		{\ensuremath{\mathit{iri}(#1)}}
\newcommand{\vterm}			[1]		{\ensuremath{\mathit{vterm}(#1)}}
\newcommand{\fedC}{\ensuremath{\bar{\calC}}}
\newcommand{\fedG}{\ensuremath{\bar\calG}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\modelsfed}	{\models_\mathit{fed}}
\newcommand{\fednew}			[2]		{\ensuremath{\mathit{fed}_{#1}(#2)}}

\newcommand{\SERVICE} {\ourStyle{SERVICE}\xspace}
\newcommand{\AND} {\ourStyle{AND}\xspace} 

\newcommand{\g} {\ensuremath{G}} %graph notation
\newcommand{\pg} {\ensuremath{\mathcal{G}}} %incomplete data source notation
\newcommand{\gs} {\ensuremath{\bar{G}}} %graph space notation
\newcommand{\pgs} {\ensuremath{\bar{\mathcal{G}}}} %partial graph space notation
\newcommand{\gc} {\ensuremath{C}} %a single gc statement
\newcommand{\gcs} {\ensuremath{\mathcal{C}}} %a set of gc statements' notation
\newcommand{\fgcs} {\ensuremath{\dot{\mathcal{C}}}} %federated gc statements (federation of fc statements) notation
\newcommand{\pgsIdeal} {\ensuremath{\dot{\mathcal{G}}^i}}

% creation of a new counter, by http://www.latex-community.org/forum/viewtopic.php?f=46&t=7587
\newcounter{mycount}
% definition of the command
\newcommand\myprob[2]{%
  \stepcounter{mycount}
  \par\noindent Problem\ \themycount .\\
  {\bfseries Input}: #1\\
  {\bfseries Output}: #2\par
}

%\newcommand{\evalwithfed}	[2]		{\ensuremath{\langle\langle #1 \rangle\rangle_{#2}}}
\newcommand{\evalwithfed}	[2]		{\ensuremath{\llbracket #1 \rrbracket^{\mathit{}}_{#2}}}


% Our completeness vocabulary
%\newcommand{\Vcompl}{\mathit{Compl}}
\newcommand{\Vcompl}{\ourStyle{Completeness}}
%\newcommand{\VhasComplStmt}{\mathit{hasComplStmt}}
\newcommand{\VhasComplStmt}{\ourStyle{hasComplStmt}}
%\newcommand{\VhasPattern}{\mathit{hasPattern}}
\newcommand{\VhasPattern}{\ourStyle{hasPattern}}
%\newcommand{\VhasCondition}{\mathit{hasCondition}}
\newcommand{\VhasCondition}{\ourStyle{hasCondition}}
%\newcommand{\Vsubject}{\mathit{subject}}
\newcommand{\Vsubject}{\ourStyle{subject}}
%\newcommand{\Vpredicate}{\mathit{predicate}}
\newcommand{\Vpredicate}{\ourStyle{predicate}}
%\newcommand{\Vobject}{\mathit{object}}
\newcommand{\Vobject}{\ourStyle{object}}
\newcommand{\VspinVarName}{\ourStyle{spin:varName}}
\newcommand{\VvarName}{\ourStyle{varName}}

% identifiers for data sources
\newcommand{\dbp} {\mathit{dbp}}

==> source_iswc/macros_iswc_-_Copy.tex <==


% This switches the style of most operators
%\newcommand{\ourStyle}[1]{{\small\texttt{#1}}}
\newcommand{\ourStyle}[1]{{\small\texttt{#1}}}



	\newcommand{\tuple}[1]{\langle\texttt{#1}\rangle} %Defines triples
	\newcommand{\ur}{\texttt{u}} % a URI
	\newcommand{\G}{{\mathcal G}} % defines an RDF graph
	%
	%Convention: sets are named by using double letters 
	\newcommand{\UU}{{\mathcal U}} % defines the set of URIs
	\newcommand{\LL}{{\mathcal L}} % defines the set of Literals
	\newcommand{\BB}{{\mathcal B}} % defines the set of Blank node ids
	
	
	\newcommand{\TC}{T_\gcs}
\newcommand{\frozen}[1]{\tilde #1}
\newcommand{\widefrozen}[1]{\widetilde #1}
\newcommand{\ID}{\mathit{id}}
\newcommand{\T}{{\cal T}}
\newcommand{\frozenID}{\frozen \ID}
\renewcommand{\C}{{\cal C}}



\newcommand{\corner}{{\tt{CoRNER}}}
\newcommand{\void}{{\tt{VoID}}}


%%%%%%%%%%%%% Ario's Macros %%%%%%%%%%%%%


\newcommand{\itl}[1]{\textit{#1}}
\newcommand{\bo}[1]{\textbf{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\bi}[1]{\textbf{\textit{#1}}}
\newcommand{\m}[1]{\boldmath{\( #1 \)}}
%\newcommand{\code}[1]{{\ttfamily #1}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\rarw}{\rightarrow}
\newcommand{\ld}{\lambda}
\newcommand{\rw}{\rightarrow}
\newcommand{\ml}{\mathcal}

\newcommand{\sq}{\hbox{$\sqcap$\llap{$\sqcup$}}}
\newcommand{\lbsq}{\hbox{\rlap{$\blacksquare$}}}

%fariz added this
\newcommand{\leftouterjoin}{\; \includegraphics[scale=0.8]{ljoin.eps} \;}

%%%%%%%%%%%%% Simon's Macros %%%%%%%%%%%%%


\global\long\def\mytpl#1{\langle#1\rangle}
\global\long\def\fc{f_{\C}}
\global\long\def\uk{\mathrm{uk}}
\global\long\def\na{\mathrm{n/a}}
\global\long\def\const{\mathrm{const}}
\global\long\def\codd{\mathrm{Codd}}
\global\long\def\sql{\mathrm{SQL}}
\global\long\def\can{\mathrm{can}}
\global\long\def\sred{\mathrm{sred}}
\global\long\def\complsred#1{\mathit{Compl^{\sred}}(#1)}
\global\long\def\complb#1{\mathit{Compl^{b}}(#1)}
\global\long\def\compls#1{\mathit{Compl^{s}}(#1)}
\global\long\def\complstar#1#2{\mathit{Compl}^{#2}(#1)}
\global\long\def\smixed{\mathrm{s+}}
\global\long\def\pdb{\mathcal{D}}
\global\long\def\domby{\preceq}
\global\long\def\dominates{\succeq}
\global\long\def\tpl#1{\bar{#1}}
\global\long\def\ctle{\mathbf{E}}
\global\long\def\ctlf{\mathbf{F}}
\global\long\def\ctla{\mathbf{A}}
\global\long\def\ctlg{\mathbf{G}}
\global\long\def\muexists{<\negthickspace\negthinspace-\negthickspace\negthinspace>}
\global\long\def\muall{[\negthinspace-\negthinspace]}
\global\long\def\mulp{\mu\mathcal{L_{\mathit{P}}}}
\global\long\def\mula{\mu\mathcal{L_{\mathit{A}}}}
\global\long\def\live{\mathrm{Live}}
\global\long\def\chase{\mathrm{chase}}
\renewcommand{\student}{\ensuremath{\mathtt{student}}\xspace}
\renewcommand{\name}{\ensuremath{\mathtt{name}}\xspace}
\renewcommand{\profile}{\ensuremath{\mathtt{profile}}\xspace}
\renewcommand{\formTeacher}{\ensuremath{\mathtt{formTeacher}}\xspace}

%---------------------------------------------------------------------------------
% MACROS FOR QUERY COMPLETENESS OVER LINKED DATA
%---------------------------------------------------------------------------------

\newcommand{\mathSet}[1]{\ensuremath{\{\,#1\,\}}}

\newcommand{\Ga}{\ensuremath{G^a}} 							% available graph
\newcommand{\Gi}{\ensuremath{G^i}} 							% ideal/complete graph

\newcommand{\QC}{\ensuremath{\mathit{Compl}(Q)}} 		% QC statement in general

\newcommand{\buildQC}[1]{\ensuremath{\mathit{Compl}(\mathit{#1})}}
\newcommand{\buildQCset}[1]{\ensuremath{\mathit{Compl}^s(\mathit{#1})}}
\newcommand{\buildQCbag}[1]{\ensuremath{\mathit{Compl}^b(\mathit{#1})}}

\newcommand{\defineGC}[2]{\ensuremath{\mathit{Compl}(#1 \mid #2)}}
\newcommand{\defineGCone}[1]{\ensuremath{\mathit{Compl}(#1)}}

\newcommand{\buildGC}[2]{\ensuremath{\mathit{Compl}(\set{#1} \mid \set{#2})}}
\newcommand{\buildGCone}[1]{\ensuremath{\mathit{Compl}(\set{#1})}}

\newcommand{\calC}{\ensuremath{\mathcal{C}}} 				% used to represent a set of GC statements
\newcommand{\GCC}{\calC} 	

\newcommand{\term}[1]{\ensuremath{\mathtt{#1}}}

\newcommand\mytabs{\hspace*{2\parindent}\=\hspace{1cm}\=\hspace{1cm}\=\hspace{1cm}\=\hspace{1cm}}
\newenvironment{mytabbing}[1][\mytabs]
  {\begin{tabbing}#1\kill}
  {\end{tabbing}}

% all SPARQL queries builder
\newcommand{\defineASK}[1]			{\ensuremath{(\ourStyle{ASK} \; #1)}}
\newcommand{\buildASK}[1]			{\ensuremath{(\ourStyle{ASK} \; \mathSet{#1})}}
\newcommand{\defineSELECT}[2]		{\ensuremath{(\ourStyle{SELECT} \; #1 \; #2)}}
\newcommand{\buildSELECT}[2]		{\ensuremath{(\ourStyle{SELECT} \; \mathSet{#1} \; \mathSet{#2})}}
\newcommand{\defineCONSTRUCT}[2]	{\ensuremath{(\ourStyle{CONSTRUCT} \; #1 \; #2)}}
\newcommand{\buildCONSTRUCT}[2]		{\ensuremath{(\ourStyle{CONSTRUCT} \; \{\mathSet{#1}\} \; \{\mathSet{#2}\})}}

\newcommand{\ASK}			{\ourStyle{ASK}\xspace}
\newcommand{\SELECT}		{\ourStyle{SELECT}\xspace}
\newcommand{\CONSTRUCT}		{\ourStyle{CONSTRUCT}\xspace}
\newcommand{\DISTINCT}		{\ourStyle{DISTINCT}\xspace}
\newcommand{\UNION}		{\ourStyle{UNION}\xspace}
\newcommand{\FILTER}	{\ourStyle{FILTER}\xspace}
\newcommand{\OR}	{\ourStyle{OR}\xspace}
\newcommand{\MINUS}	{\ourStyle{MINUS}\xspace}


\newcommand{\map}[2]{\ensuremath{\text{#1} \mapsto \text{#2}}}
\newcommand{\triple}[3]{(\mathit{#1}, \mathit{#2}, \mathit{#3})}

\newcommand{\buildIFF}[2]{\ensuremath{#1 \;\;\;\; \text{iff} \;\;\;\; #2}}

\newcommand{\evalset}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}^s}}
\newcommand{\evalbag}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}^b}}
\newcommand{\evalsetbag}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}}}
\newcommand{\eval}	[2]		{\ensuremath{\llbracket #1 \rrbracket_{#2}}}
\newcommand{\cardMapping}	[2]		{\ensuremath{\mathit{card}_{#1}(#2)}}						%1: mapping bag, 2: mapping

\newcommand{\vars}[1]{\ensuremath{\mathit{vars}(#1)}}

% macros w/o parameters
\newcommand{\emptymap}		{\ensuremath{\mu_{\emptyset}}}
\newcommand{\mappingset}	{\ensuremath{\Omega}}
\newcommand{\rhodf}			{\ensuremath{\rho \mathit{DF}}}
\newcommand{\cl}				{\ensuremath{\mathit{cl}}}
\newcommand{\alphaVersion} 	{{\color{red} ALPHA VERSION!!!}}


\newcommand{\Graph}{\ensuremath{G}}
\newcommand{\Pattern}{\ensuremath{P}}

% DB stuff
\newcommand{\buildDBQuery}[2]{\ensuremath{{#1}\;\text{:-}\;{#2}}}

% federated query stuff
\newcommand{\calF}{\ensuremath{\mathcal{F}}} 				% used to represent a set of data sources
\newcommand{\fed}			[1]		{\ensuremath{\mathit{fed}_\calF(#1)}}
\newcommand{\evalfed}	[2]		{\ensuremath{\llbracket \fed{#1} \rrbracket_{#2}^s}}
\newcommand{\evalfedset}	[1]		{\ensuremath{\llbracket \fed{#1} \rrbracket_{\emptyset}^s}}
\newcommand{\defineSERVICE}[2]		{\ensuremath{(\ourStyle{SERVICE} \; #1 \; #2)}}

% OPT stuff
\newcommand{\subsumedBy}{\sqsubseteq}
\newcommand{\lessInformativeThan}{\subsumedBy}
\newcommand{\buildSELECTnew}[2]		{\ensuremath{(\mathit{SELECT} \; \mathSet{#1} \; #2)}}
%\newcommand{\OPT} {$\;$ OPT $\;$}
\newcommand{\newvars}			[1]		{\ensuremath{\mathit{newvars}(#1)}}
\newcommand{\ext}			[1]		{\ensuremath{\mathit{ext}(#1)}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}} 				% used to represent trees

\newcommand{\evaltopdown}	[2]		{\ensuremath{\llbracket #1 \rrbracket^{td}_{#2}}}

% QUERY GENERATOR
\newcommand{\queryMINUS} [2] {(#1 \ourStyle{ MINUS } #2)}
\newcommand{\queryUNION} [2] {(#1 \ourStyle{ UNION } #2)}
\newcommand{\queryAND} [2] {(#1 \ourStyle{ AND } #2)}
\newcommand{\queryOPT} [2] {(#1 \ourStyle{ OPT } #2)}
\newcommand{\queryFILTER} [2] {(#1 \ourStyle{ FILTER } #2)}
\newcommand{\querySERVICE} [2] {(\ourStyle{SERVICE} \; #1 \; #2)}
\newcommand{\querySERVICEBraces} [2] {(\ourStyle{SERVICE} \; #1 \; \{#2\})}


\newcommand{\yes} {\texttt{yes}}
\newcommand{\notexists}	[1]	{\ensuremath{\ourStyle{NOT} \; \ourStyle{EXISTS}}(#1)}

\newcommand{\iri}			[1]		{\ensuremath{\mathit{iri}(#1)}}
\newcommand{\vterm}			[1]		{\ensuremath{\mathit{vterm}(#1)}}
\newcommand{\fedC}{\ensuremath{\bar{\calC}}}
\newcommand{\fedG}{\ensuremath{\bar\calG}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\modelsfed}	{\models_\mathit{fed}}
\newcommand{\fednew}			[2]		{\ensuremath{\mathit{fed}_{#1}(#2)}}

\newcommand{\SERVICE} {\ourStyle{SERVICE}\xspace}
\newcommand{\AND} {\ourStyle{AND}\xspace} 

\newcommand{\g} {\ensuremath{G}} %graph notation
\newcommand{\pg} {\ensuremath{\mathcal{G}}} %incomplete data source notation
\newcommand{\gs} {\ensuremath{\bar{G}}} %graph space notation
\newcommand{\pgs} {\ensuremath{\bar{\mathcal{G}}}} %partial graph space notation
\newcommand{\gc} {\ensuremath{C}} %a single gc statement
\newcommand{\gcs} {\ensuremath{\mathcal{C}}} %a set of gc statements' notation
\newcommand{\fgcs} {\ensuremath{\dot{\mathcal{C}}}} %federated gc statements (federation of fc statements) notation
\newcommand{\pgsIdeal} {\ensuremath{\dot{\mathcal{G}}^i}}

% creation of a new counter, by http://www.latex-community.org/forum/viewtopic.php?f=46&t=7587
\newcounter{mycount}
% definition of the command
\newcommand\myprob[2]{%
  \stepcounter{mycount}
  \par\noindent Problem\ \themycount .\\
  {\bfseries Input}: #1\\
  {\bfseries Output}: #2\par
}

%\newcommand{\evalwithfed}	[2]		{\ensuremath{\langle\langle #1 \rangle\rangle_{#2}}}
\newcommand{\evalwithfed}	[2]		{\ensuremath{\llbracket #1 \rrbracket^{\mathit{}}_{#2}}}


% Our completeness vocabulary
%\newcommand{\Vcompl}{\mathit{Compl}}
\newcommand{\Vcompl}{\ourStyle{Completeness}}
%\newcommand{\VhasComplStmt}{\mathit{hasComplStmt}}
\newcommand{\VhasComplStmt}{\ourStyle{hasComplStmt}}
%\newcommand{\VhasPattern}{\mathit{hasPattern}}
\newcommand{\VhasPattern}{\ourStyle{hasPattern}}
%\newcommand{\VhasCondition}{\mathit{hasCondition}}
\newcommand{\VhasCondition}{\ourStyle{hasCondition}}
%\newcommand{\Vsubject}{\mathit{subject}}
\newcommand{\Vsubject}{\ourStyle{subject}}
%\newcommand{\Vpredicate}{\mathit{predicate}}
\newcommand{\Vpredicate}{\ourStyle{predicate}}
%\newcommand{\Vobject}{\mathit{object}}
\newcommand{\Vobject}{\ourStyle{object}}
\newcommand{\VspinVarName}{\ourStyle{spin:varName}}
\newcommand{\VvarName}{\ourStyle{varName}}

% identifiers for data sources
\newcommand{\dbp} {\mathit{dbp}}

==> source_vldb/texfiles/abstract.tex <==
\begin{abstract}




\end{abstract}

% 	\category{X.Y}{Something General}{Something Less General}[Something better described]
% 	\category{Z.W}{Something Else}{Something Else General}[Something else better described]
% 	\terms{something \& anything}
% 	\keywords{Semantic Web, Cloud Computing, Ontologies, Web 3.0, Ubiquitous Mobile Devices}




==> source_vldb/texfiles/acknowledgement.tex <==
\subsubsection*{Acknowledgement}

We are thankful to Zeno Moriggl and Martin Prosch from the school IT
department of the province of Bolzano for introducing us to their
problem of query completeness  and to Dmitrijs Milajevs for having explored this problem in his BSc thesis.
We thank Balder ten Cate and Leonid Libkin for pointing out important
connections to our work.
This work has been partially supported by the project ACSI, funded by the EU under FP7 grant agreement n. 257593.

==> source_vldb/texfiles/bibliography.tex <==
\bibliography{completeness}
%\bibliographystyle{alpha}
\bibliographystyle{abbrv}

==> source_vldb/texfiles/environments.tex <==
%%%\newtheorem{theorem}{Theorem}[section]
%%%\newtheorem{lemma}[theorem]{Lemma}
%%%\newtheorem{proposition}[theorem]{Proposition}
%%%\newtheorem{corollary}[theorem]{Corollary}

%\theoremstyle{definition}

%%%\newtheorem{example}[theorem]{Example}



%\renewenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}


%\theoremstyle{plain}% default

% \newdef{example}{Example}
 
%\newenvironment{nonumberlemma}
%{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries}]}{\end{trivlist}}

%\newenvironment{nonumberlemma}
%{\rule{1ex}{1ex}\hspace{\stretch{1}}}
%{\hspace{\stretch{1}}\rule{1ex}{1ex}}


% \newdef{nonumberlemma}{Lemma} 
 
% \newtheorem*{nonumberlemma}{Lemma}
 
% \theoremstyle{definition}
% \newtheorem{example}[theorem]{Example}

%\newtheorem{example}[theorem]{Example}
%\renewenvironment{example}[1][Example]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}



==> source_vldb/texfiles/formalization.tex <==




==> source_vldb/texfiles/related_work.tex <==




==> source_vldb/texfiles/title.tex <==
\title{Completeness of Queries over Incomplete Databases}
%\conferenceinfo{VLDB 2011}{Seattle, USA}
%\CopyrightYear{2011}


\numberofauthors{2}
\author{
\alignauthor Simon Razniewski\\
		\affaddr{\hspace*{-.7cm}\makebox{Free University of
Bozen-Bolzano}}\\
		\affaddr{Dominikanerplatz 3}\\
		\affaddr{39100 Bozen, Italy}\\
		\email{razniewski@inf.unibz.it}
\alignauthor Werner Nutt\\
		\affaddr{\hspace*{-.7cm}\makebox{Free University of
Bozen-Bolzano}}\\
		\affaddr{Dominikanerplatz 3}\\
		\affaddr{39100 Bozen, Italy}\\
		\email{nutt@inf.unibz.it}
}
